CausalSim: A Causal Framework for Unbiased Trace-Driven Simulation

We present CausalSim, a causal framework for unbiased trace-driven simulation. Current trace-driven simulators assume that the interventions being simulated (e.g., a new algorithm) would not affect the validity of the traces. However, real-world traces are often biased by the choices algorithms make during trace collection, and hence replaying traces under an intervention may lead to incorrect results. CausalSim addresses this challenge by learning a causal model of the system dynamics and latent factors capturing the underlying system conditions during trace collection. It learns these models using an initial randomized control trial (RCT) under a fixed set of algorithms, and then applies them to remove biases from trace data when simulating new algorithms. Key to CausalSim is mapping unbiased trace-driven simulation to a tensor completion problem with extremely sparse observations. By exploiting a basic distributional invariance property present in RCT data, CausalSim enables a novel tensor completion method despite the sparsity of observations. Our extensive evaluation of CausalSim on both real and synthetic datasets, including more than ten months of real data from the Puffer video streaming system shows it improves simulation accuracy, reducing errors by 53% and 61% on average compared to expert-designed and supervised learning baselines. Moreover, CausalSim provides markedly different insights about ABR algorithms compared to the biased baseline simulator, which we validate with a real deployment.

==> figures/raw_data/abr_rl/cdf_full_v1.tex <==

\addplot[solid, black, thick, mark=none] coordinates{
(0.190998240493362, 0.003125)
(0.33872490363070323, 1.003125)
(0.38974581450243007, 2.003125)
(0.42573814845339986, 3.003125)
(0.45715507193126537, 4.003125)
(0.4849078410947504, 5.003125)
(0.5080800047895916, 6.003125)
(0.5287578842582081, 7.003125000000001)
(0.5463307121131012, 8.003125)
(0.5643557565587533, 9.003124999999999)
(0.5845121296100694, 10.003125)
(0.5993330704985171, 11.003124999999999)
(0.6129857870186345, 12.003125)
(0.6266595796903425, 13.003124999999999)
(0.6403930990726566, 14.003124999999999)
(0.6541373262749988, 15.003125)
(0.669305741435975, 16.003125)
(0.682075383850339, 17.003125)
(0.6950813598107943, 18.003125)
(0.7064890675540104, 19.003125)
(0.7175832402491157, 20.003125)
(0.7296518901997748, 21.003125)
(0.7412026620371363, 22.003125)
(0.75262242529309, 23.003125)
(0.7649620583842079, 24.003125)
(0.776941300733881, 25.003124999999997)
(0.7886888940701979, 26.003125)
(0.8003332816447523, 27.003125)
(0.8120090508105254, 28.003125)
(0.8242461227249925, 29.003125)
(0.8350781128854089, 30.003125000000004)
(0.8479313156658127, 31.003124999999997)
(0.8622322997574322, 32.003125)
(0.8761883757717602, 33.003125)
(0.8892690112830968, 34.003125)
(0.9011334036676119, 35.003125000000004)
(0.9140167507109814, 36.003125000000004)
(0.9282893483075262, 37.003125)
(0.9421072123762846, 38.003125)
(0.9555725934317582, 39.003125)
(0.9685354941884757, 40.003125)
(0.9814725734140215, 41.003125000000004)
(0.994401698408036, 42.003125000000004)
(1.0083463175130385, 43.003125)
(1.0209865860909495, 44.003125)
(1.0343325080426597, 45.003125)
(1.04830651801412, 46.003125)
(1.0615712892862479, 47.003125000000004)
(1.074598104033273, 48.003125000000004)
(1.088829356945474, 49.003125)
(1.1031781162430854, 50.003125000000004)
(1.117039863969929, 51.003125000000004)
(1.1324135793765921, 52.003125)
(1.147569340085269, 53.003125)
(1.1613526753924805, 54.003125)
(1.1756673507022544, 55.003125)
(1.1897715983478394, 56.003125)
(1.2041951609837533, 57.003125)
(1.2215908045851394, 58.003125)
(1.2373805555857216, 59.003125)
(1.2534291029737623, 60.003125000000004)
(1.2690487724292003, 61.003125000000004)
(1.2853395674361443, 62.003125000000004)
(1.3022231902874628, 63.003125000000004)
(1.3193244748802342, 64.00312500000001)
(1.3359904244549738, 65.003125)
(1.3528616628729417, 66.003125)
(1.3710933904332983, 67.003125)
(1.388814067225557, 68.003125)
(1.4082479902994447, 69.003125)
(1.425220957938314, 70.003125)
(1.4456967770162947, 71.003125)
(1.4663767741618199, 72.003125)
(1.4883993994512006, 73.003125)
(1.5099739741673148, 74.003125)
(1.5334048702663357, 75.003125)
(1.555519056983489, 76.00312500000001)
(1.580800191734968, 77.003125)
(1.6031270010144245, 78.003125)
(1.6249904996034261, 79.003125)
(1.6499678645994558, 80.003125)
(1.6753830594103132, 81.003125)
(1.7031756096746336, 82.003125)
(1.7263428685239934, 83.003125)
(1.7533485129024076, 84.003125)
(1.7823789591964794, 85.003125)
(1.811924908236433, 86.003125)
(1.84275699190578, 87.003125)
(1.8794202015259431, 88.00312500000001)
(1.9129218002816033, 89.00312500000001)
(1.9526292034848702, 90.003125)
(1.9945313242732425, 91.003125)
(2.0375961759560197, 92.003125)
(2.089991176763295, 93.003125)
(2.1470562749327886, 94.003125)
(2.2152765054558463, 95.003125)
(2.285052633268245, 96.003125)
(2.3677263264827695, 97.003125)
(2.4684897666807806, 98.003125)
(2.612885046436263, 99.003125)
};
\addplot[solid, green!70!black, thick, mark=none] coordinates{
(-0.42688482564518077, 0.003125)
(0.20051326215781165, 1.003125)
(0.28290820430169084, 2.003125)
(0.33502011008503757, 3.003125)
(0.3771667060533893, 4.003125)
(0.41080638659143415, 5.003125)
(0.44262941313501364, 6.003125)
(0.4701666237737582, 7.003125000000001)
(0.49678657252467895, 8.003125)
(0.5189111024871964, 9.003124999999999)
(0.5396324349297543, 10.003125)
(0.5591394340388389, 11.003124999999999)
(0.5788276890547444, 12.003125)
(0.5973297588017085, 13.003124999999999)
(0.6131725851938831, 14.003124999999999)
(0.6263411106185439, 15.003125)
(0.6415285922762746, 16.003125)
(0.6564635436031017, 17.003125)
(0.6721042250428368, 18.003125)
(0.6865829532805418, 19.003125)
(0.698999145629, 20.003125)
(0.7097054010237793, 21.003125)
(0.7230243707863585, 22.003125)
(0.7359056599979015, 23.003125)
(0.7478752647133329, 24.003125)
(0.760390932570382, 25.003124999999997)
(0.7728727573665081, 26.003125)
(0.7856319190465482, 27.003125)
(0.7979286477489242, 28.003125)
(0.8085357515643362, 29.003125)
(0.8212905886667772, 30.003125000000004)
(0.83395972493353, 31.003124999999997)
(0.8486351013211886, 32.003125)
(0.8637465248268004, 33.003125)
(0.8771106609028193, 34.003125)
(0.88975827677771, 35.003125000000004)
(0.9031561380696157, 36.003125000000004)
(0.9185625230069244, 37.003125)
(0.9331646194749915, 38.003125)
(0.9472611927537907, 39.003125)
(0.9611533657815908, 40.003125)
(0.9746945674662822, 41.003125000000004)
(0.9876367207528249, 42.003125000000004)
(0.9990772376923346, 43.003125)
(1.0125032695675382, 44.003125)
(1.026205898961052, 45.003125)
(1.04061138863604, 46.003125)
(1.0555508811229826, 47.003125000000004)
(1.0689959405920912, 48.003125000000004)
(1.081611612172751, 49.003125)
(1.0955954013118627, 50.003125000000004)
(1.109704561677818, 51.003125000000004)
(1.1232135451285912, 52.003125)
(1.1366809571298706, 53.003125)
(1.1525250873549047, 54.003125)
(1.1650408621198791, 55.003125)
(1.1784833652139906, 56.003125)
(1.1930675942373468, 57.003125)
(1.208983639329546, 58.003125)
(1.2247803557485903, 59.003125)
(1.2406586377503666, 60.003125000000004)
(1.256441721750232, 61.003125000000004)
(1.2728613839203715, 62.003125000000004)
(1.2895372761527002, 63.003125000000004)
(1.3056023907615786, 64.00312500000001)
(1.3233187418644436, 65.003125)
(1.3401609539885062, 66.003125)
(1.3585193921911474, 67.003125)
(1.3754245764728965, 68.003125)
(1.3923806401559102, 69.003125)
(1.4118863588400818, 70.003125)
(1.4301239235453964, 71.003125)
(1.4508062214810302, 72.003125)
(1.4729949190980207, 73.003125)
(1.4942916810470692, 74.003125)
(1.5182861333996502, 75.003125)
(1.541469899540271, 76.00312500000001)
(1.563387837994101, 77.003125)
(1.585632740969034, 78.003125)
(1.6094524827769192, 79.003125)
(1.6313813783832292, 80.003125)
(1.656056496854128, 81.003125)
(1.6821893784695434, 82.003125)
(1.7057397320720333, 83.003125)
(1.7332538372045028, 84.003125)
(1.7593948316618722, 85.003125)
(1.7899387094476638, 86.003125)
(1.8196884312304282, 87.003125)
(1.848943362736331, 88.00312500000001)
(1.8837477396853748, 89.00312500000001)
(1.921141100643219, 90.003125)
(1.9626157593244553, 91.003125)
(2.006791131456998, 92.003125)
(2.0579791980883497, 93.003125)
(2.1173350567595475, 94.003125)
(2.1865386976461596, 95.003125)
(2.260369244078304, 96.003125)
(2.344232988027499, 97.003125)
(2.4527427887016184, 98.003125)
(2.6003077282197555, 99.003125)
};
\addplot[solid, blue, thick, mark=none] coordinates{
(0.246434974802348, 0.003125)
(0.2668844874452027, 1.003125)
(0.26823257588496263, 2.003125)
(0.26896457411249725, 3.003125)
(0.2695538753476837, 4.003125)
(0.26997224685159354, 5.003125)
(0.2703587749551739, 6.003125)
(0.27077340242949083, 7.003125000000001)
(0.2714031931548458, 8.003125)
(0.272148782777021, 9.003124999999999)
(0.27289100223221474, 10.003125)
(0.27374197424360547, 11.003124999999999)
(0.2759990288981496, 12.003125)
(0.3006074084413234, 13.003124999999999)
(0.3347192892341421, 14.003124999999999)
(0.3702513021600811, 15.003125)
(0.4031838595076532, 16.003125)
(0.43717450501641714, 17.003125)
(0.46692753723257363, 18.003125)
(0.5010455318858407, 19.003125)
(0.5290338314511324, 20.003125)
(0.551902201576835, 21.003125)
(0.5795109846743369, 22.003125)
(0.6028514887202753, 23.003125)
(0.6252866092978434, 24.003125)
(0.6468868735985623, 25.003124999999997)
(0.6671624377665594, 26.003125)
(0.686077637666003, 27.003125)
(0.7032218352560741, 28.003125)
(0.7173425703028835, 29.003125)
(0.7355027354142625, 30.003125000000004)
(0.7533002750153074, 31.003124999999997)
(0.771101881338926, 32.003125)
(0.7895613451821804, 33.003125)
(0.806087003318646, 34.003125)
(0.8232053309864522, 35.003125000000004)
(0.8402866117814023, 36.003125000000004)
(0.8579050460305496, 37.003125)
(0.8754026483878556, 38.003125)
(0.8934385212235303, 39.003125)
(0.9108156195496966, 40.003125)
(0.925291274327382, 41.003125000000004)
(0.9401949014606281, 42.003125000000004)
(0.9565162196334326, 43.003125)
(0.9725702233356508, 44.003125)
(0.9870807867481582, 45.003125)
(1.0025084438664358, 46.003125)
(1.0183293751218192, 47.003125000000004)
(1.0327604969826738, 48.003125000000004)
(1.0479397981058047, 49.003125)
(1.0635425905303484, 50.003125000000004)
(1.079164589033711, 51.003125000000004)
(1.0929058808980348, 52.003125)
(1.107304534202403, 53.003125)
(1.1233515054493861, 54.003125)
(1.1367005441906086, 55.003125)
(1.1516537208118336, 56.003125)
(1.1660262050725299, 57.003125)
(1.1811387454859759, 58.003125)
(1.1984403372246142, 59.003125)
(1.216924997763661, 60.003125000000004)
(1.2339286188665364, 61.003125000000004)
(1.2529307325512862, 62.003125000000004)
(1.2710304448379512, 63.003125000000004)
(1.2898698880242827, 64.00312500000001)
(1.3078123800640367, 65.003125)
(1.3244077006451875, 66.003125)
(1.3418024801086101, 67.003125)
(1.3598911569323335, 68.003125)
(1.3786632010393993, 69.003125)
(1.398309654491639, 70.003125)
(1.4202031282831646, 71.003125)
(1.4418222685725317, 72.003125)
(1.46509561515087, 73.003125)
(1.4882117151664864, 74.003125)
(1.5108818163612363, 75.003125)
(1.532001283663327, 76.00312500000001)
(1.5552735961607629, 77.003125)
(1.579805149554475, 78.003125)
(1.6050978954784425, 79.003125)
(1.6277805724232852, 80.003125)
(1.652748168852754, 81.003125)
(1.6771311492300904, 82.003125)
(1.7025895621699818, 83.003125)
(1.7276551392364772, 84.003125)
(1.7568293372719554, 85.003125)
(1.7889999227488695, 86.003125)
(1.818606967563438, 87.003125)
(1.848814152406382, 88.00312500000001)
(1.885268618293127, 89.00312500000001)
(1.9200817297611406, 90.003125)
(1.9622727646147566, 91.003125)
(2.0112026492540283, 92.003125)
(2.06056293199403, 93.003125)
(2.1217985196227747, 94.003125)
(2.1843807434096596, 95.003125)
(2.2611706777750795, 96.003125)
(2.349411272036801, 97.003125)
(2.4527733429489373, 98.003125)
(2.6019346229270144, 99.003125)
};
\addplot[solid, red, thick, mark=none] coordinates{
(0.1876539715536661, 0.003125)
(0.26734285363814053, 1.003125)
(0.2686096154540846, 2.003125)
(0.2692326474384404, 3.003125)
(0.2697301477551018, 4.003125)
(0.2699746309418502, 5.003125)
(0.2702691596705297, 6.003125)
(0.2705467622917848, 7.003125000000001)
(0.27094282462170605, 8.003125)
(0.2714700745317645, 9.003124999999999)
(0.2726239161859334, 10.003125)
(0.28373529563633915, 11.003124999999999)
(0.3052473367846221, 12.003125)
(0.33390342448332044, 13.003124999999999)
(0.36381518867932827, 14.003124999999999)
(0.3936852193398359, 15.003125)
(0.42245624291589584, 16.003125)
(0.4538793188838214, 17.003125)
(0.486766341751111, 18.003125)
(0.5158262207114365, 19.003125)
(0.5422645993329125, 20.003125)
(0.5654658013828251, 21.003125)
(0.5906434564129149, 22.003125)
(0.6128584026775558, 23.003125)
(0.6338072560015696, 24.003125)
(0.6556085235182919, 25.003124999999997)
(0.675524137205716, 26.003125)
(0.6917695664115489, 27.003125)
(0.7055829963198706, 28.003125)
(0.7204821970906067, 29.003125)
(0.7384491453570634, 30.003125000000004)
(0.7564288624247403, 31.003124999999997)
(0.77570609663584, 32.003125)
(0.7932675250362605, 33.003125)
(0.8101111372280474, 34.003125)
(0.8271128305108204, 35.003125000000004)
(0.8452876974502017, 36.003125000000004)
(0.8633711188368001, 37.003125)
(0.8799920647857086, 38.003125)
(0.8971448639901438, 39.003125)
(0.9141895115171021, 40.003125)
(0.9290733730824975, 41.003125000000004)
(0.9433814402351488, 42.003125000000004)
(0.9586176403000735, 43.003125)
(0.9731108525648449, 44.003125)
(0.9891556600060322, 45.003125)
(1.0033698748856668, 46.003125)
(1.0175852488693193, 47.003125000000004)
(1.0319318358181422, 48.003125000000004)
(1.0469440663631577, 49.003125)
(1.0608465516426908, 50.003125000000004)
(1.0773722093043194, 51.003125000000004)
(1.0911037451490997, 52.003125)
(1.1041967146542573, 53.003125)
(1.1184420591663857, 54.003125)
(1.1323418385281374, 55.003125)
(1.1473597130943922, 56.003125)
(1.161659123958662, 57.003125)
(1.1748276731372702, 58.003125)
(1.191898854142639, 59.003125)
(1.2090427012652796, 60.003125000000004)
(1.2262190955068797, 61.003125000000004)
(1.2433220862833456, 62.003125000000004)
(1.2599334464095344, 63.003125000000004)
(1.2778424161586872, 64.00312500000001)
(1.296777120422776, 65.003125)
(1.3148154260922829, 66.003125)
(1.3315240434603859, 67.003125)
(1.3488886790005616, 68.003125)
(1.3671084872876218, 69.003125)
(1.3866764588877107, 70.003125)
(1.4056903326142973, 71.003125)
(1.4271011369127997, 72.003125)
(1.4485246576155424, 73.003125)
(1.4702908488326076, 74.003125)
(1.4935814014780693, 75.003125)
(1.5143476464863657, 76.00312500000001)
(1.534847764924859, 77.003125)
(1.5608722493517662, 78.003125)
(1.5845620867535493, 79.003125)
(1.6085114275954437, 80.003125)
(1.6333892872359512, 81.003125)
(1.6594486098969172, 82.003125)
(1.6820008074206847, 83.003125)
(1.7080415755524987, 84.003125)
(1.7366201353706292, 85.003125)
(1.7673128304204648, 86.003125)
(1.7981727204377973, 87.003125)
(1.8278474745714512, 88.00312500000001)
(1.8609288654829053, 89.00312500000001)
(1.8985115108269703, 90.003125)
(1.9384678939553304, 91.003125)
(1.9879413781330817, 92.003125)
(2.040708141129679, 93.003125)
(2.1009278344647484, 94.003125)
(2.1660614063802144, 95.003125)
(2.2448967258930974, 96.003125)
(2.332932142549276, 97.003125)
(2.4446100776428152, 98.003125)
(2.596473395496708, 99.003125)
};
\addplot[solid, magenta, thick, mark=none] coordinates{
(-0.44908520044703865, 0.0125)
(0.08634244740145001, 1.0125)
(0.14214849229604856, 2.0125)
(0.18813115315219814, 3.0124999999999997)
(0.2252282816214521, 4.0125)
(0.2556486806505378, 5.0125)
(0.28472597394667126, 6.0125)
(0.3135294908987421, 7.012500000000001)
(0.3411652987081591, 8.0125)
(0.36297794039836306, 9.0125)
(0.38294941559893114, 10.012500000000001)
(0.40286003976992624, 11.0125)
(0.4232510479963157, 12.0125)
(0.4415428826525561, 13.0125)
(0.4613289954963792, 14.0125)
(0.4785155898611809, 15.012500000000001)
(0.49631849623288377, 16.0125)
(0.510392395081644, 17.0125)
(0.5241471350890905, 18.0125)
(0.5360745614659829, 19.0125)
(0.5488289529381665, 20.0125)
(0.5601650926578465, 21.0125)
(0.5730302139519048, 22.0125)
(0.5835399699366284, 23.0125)
(0.5924517675016758, 24.0125)
(0.6033046071035669, 25.0125)
(0.6131074960852142, 26.0125)
(0.6217005543919311, 27.0125)
(0.6295305250706195, 28.012500000000003)
(0.6402218433285213, 29.012500000000003)
(0.6483887526826416, 30.012499999999996)
(0.6583821300022724, 31.0125)
(0.671364533424392, 32.0125)
(0.6873850560676986, 33.0125)
(0.7055138482303305, 34.0125)
(0.7212137395949272, 35.0125)
(0.7352061775300732, 36.012499999999996)
(0.7486794875803502, 37.012499999999996)
(0.764680425903991, 38.012499999999996)
(0.7812556659569561, 39.0125)
(0.7949797065267792, 40.0125)
(0.8094505444618358, 41.0125)
(0.8218750446841351, 42.0125)
(0.8369122735698675, 43.012499999999996)
(0.852182569363908, 44.012499999999996)
(0.8651896396615215, 45.0125)
(0.8770540303376432, 46.0125)
(0.88871015898527, 47.0125)
(0.904252514662866, 48.0125)
(0.9213755059573434, 49.012499999999996)
(0.9353947690076793, 50.0125)
(0.9494102501794924, 51.0125)
(0.9633373729945747, 52.012499999999996)
(0.9791628081263827, 53.012499999999996)
(0.9938686606478018, 54.012499999999996)
(1.006284161361234, 55.012499999999996)
(1.0185328004160445, 56.012499999999996)
(1.0311851223969464, 57.0125)
(1.0453770875669797, 58.0125)
(1.060492988653504, 59.0125)
(1.074514236881001, 60.0125)
(1.0935131351389566, 61.0125)
(1.1078250204587718, 62.0125)
(1.1257885453789207, 63.0125)
(1.1435200477445189, 64.0125)
(1.1590652360566986, 65.01249999999999)
(1.178808774509051, 66.0125)
(1.197629196292091, 67.0125)
(1.2203363983145428, 68.0125)
(1.2399718344664306, 69.0125)
(1.2631200292586038, 70.0125)
(1.2829089746914746, 71.0125)
(1.3003348439350308, 72.0125)
(1.325943390580877, 73.0125)
(1.3470635140620373, 74.0125)
(1.372811301285503, 75.0125)
(1.3943251874883809, 76.0125)
(1.4180857259347153, 77.01249999999999)
(1.4404174494053261, 78.01249999999999)
(1.4584776677453009, 79.0125)
(1.4812930385518197, 80.0125)
(1.5022389903353461, 81.0125)
(1.5224095903217965, 82.0125)
(1.5438414803464637, 83.0125)
(1.5603877541724955, 84.0125)
(1.5845647003647665, 85.0125)
(1.604162634181094, 86.0125)
(1.6296187081935753, 87.0125)
(1.6492175839714418, 88.0125)
(1.6690536585203175, 89.0125)
(1.6948057937701393, 90.01249999999999)
(1.7160468415637617, 91.0125)
(1.7412571750375363, 92.0125)
(1.7610244972286677, 93.0125)
(1.7827340782715686, 94.0125)
(1.8010727261124533, 95.0125)
(1.8168243018820789, 96.0125)
(1.8245360845777883, 97.0125)
(1.8288249305552589, 98.0125)
(1.8317981638838534, 99.0125)
};

==> figures/raw_data/abr_rl/cdf_high_v1.tex <==

\addplot[solid, black, thick, mark=none] coordinates{
(0.190998240493362, 0.007568876778686043)
(0.2932563824843381, 1.006660611565244)
(0.3322929974613566, 2.005752346351801)
(0.3561280841327832, 3.004844081138359)
(0.37979983514818366, 4.003935815924916)
(0.39846602677926213, 5.003027550711474)
(0.41349739866457524, 6.002119285498033)
(0.42973159774973396, 7.00121102028459)
(0.4448569492278534, 8.000302755071148)
(0.4599619992606676, 8.999394489857705)
(0.47187663120888956, 9.998486224644262)
(0.4870919124566906, 10.99757795943082)
(0.49747018312492974, 11.996669694217378)
(0.5083314047327195, 12.995761429003934)
(0.5188177411022887, 13.994853163790493)
(0.529076246888634, 14.993944898577052)
(0.5382718138204428, 15.993036633363609)
(0.5468937170216692, 16.992128368150166)
(0.5558076655489308, 17.991220102936726)
(0.5664275171724961, 18.99031183772328)
(0.575941038799325, 19.98940357250984)
(0.5861952454644946, 20.988495307296397)
(0.5944413693322789, 21.987587042082954)
(0.6008529655048647, 22.986678776869514)
(0.6082337031296566, 23.98577051165607)
(0.6148515402379167, 24.984862246442628)
(0.6214061824017971, 25.983953981229185)
(0.6281232545259093, 26.98304571601574)
(0.6348104457630762, 27.982137450802302)
(0.6427289665369531, 28.98122918558886)
(0.6493549823684706, 29.980320920375412)
(0.6569581962432307, 30.979412655161976)
(0.665910456767652, 31.97850438994853)
(0.6730063312469226, 32.977596124735086)
(0.679353807269625, 33.97668785952165)
(0.6866632104016358, 34.97577959430821)
(0.6938884560961277, 35.97487132909476)
(0.6997403996512185, 36.97396306388132)
(0.7054964865098652, 37.973054798667874)
(0.7119102980135944, 38.972146533454435)
(0.7176385406155046, 39.971238268240995)
(0.7242923487301548, 40.97033000302755)
(0.7310584109754124, 41.96942173781411)
(0.7372961709732255, 42.96851347260067)
(0.7439959880270856, 43.96760520738722)
(0.7502110104935262, 44.96669694217378)
(0.7573936167456472, 45.96578867696034)
(0.7635418407389, 46.9648804117469)
(0.7698053855138209, 47.96397214653346)
(0.7771768644914442, 48.96306388132001)
(0.7844600784600848, 49.96215561610657)
(0.7902494353404401, 50.961247350893125)
(0.7977073714570454, 51.960339085679685)
(0.8043548864814676, 52.959430820466245)
(0.8109441723164158, 53.9585225552528)
(0.8181746806768653, 54.95761429003936)
(0.825455644359045, 55.95670602482592)
(0.8326471078546164, 56.95579775961247)
(0.8407936246675871, 57.95488949439903)
(0.8483824609567049, 58.953981229185594)
(0.858019104498272, 59.95307296397214)
(0.8670148683396591, 60.95216469875871)
(0.8760632638845326, 61.95125643354527)
(0.8839625025138697, 62.950348168331814)
(0.8914713009471057, 63.949439903118375)
(0.9004912070501425, 64.94853163790494)
(0.9084380582577313, 65.94762337269148)
(0.9175303309152032, 66.94671510747806)
(0.9285048518527866, 67.94580684226462)
(0.9381486462099081, 68.94489857705116)
(0.947962993765462, 69.94399031183772)
(0.959378533615409, 70.94308204662428)
(0.9688938809280471, 71.94217378141083)
(0.9782053603562239, 72.94126551619739)
(0.9877787298763601, 73.94035725098395)
(0.9978567634466373, 74.93944898577051)
(1.00871665609285, 75.93854072055707)
(1.0197982659292508, 76.93763245534363)
(1.0311106889635027, 77.93672419013018)
(1.0431607262600717, 78.93581592491674)
(1.055694574285377, 79.9349076597033)
(1.0659300006752954, 80.93399939448986)
(1.0779447991564657, 81.93309112927642)
(1.093109431201293, 82.93218286406298)
(1.1055444325427888, 83.93127459884953)
(1.1185931774114342, 84.93036633363609)
(1.133962858005558, 85.92945806842265)
(1.1500331003119828, 86.9285498032092)
(1.165466548314635, 87.92764153799575)
(1.1797797675580943, 88.92673327278231)
(1.1960749779270252, 89.92582500756887)
(1.2149556874113983, 90.92491674235544)
(1.2359741234587927, 91.924008477142)
(1.2582362696450418, 92.92310021192854)
(1.281523898246642, 93.9221919467151)
(1.3112688749762658, 94.92128368150166)
(1.347711736313467, 95.92037541628822)
(1.395415268290078, 96.91946715107478)
(1.446750198310936, 97.91855888586134)
(1.5248397028154457, 98.9176506206479)
(1.7712067290610936, 99.91674235543445)
};
\addplot[solid, green!70!black, thick, mark=none] coordinates{
(-0.42688482564518077, 0.007568876778686043)
(0.1396037439040878, 1.006660611565244)
(0.21779104230961716, 2.005752346351801)
(0.2623795854722768, 3.004844081138359)
(0.2990530563881624, 4.003935815924916)
(0.326810889440031, 5.003027550711474)
(0.3521694377147121, 6.002119285498033)
(0.373117290681554, 7.00121102028459)
(0.3913471911172089, 8.000302755071148)
(0.4077266285716326, 8.999394489857705)
(0.42510716880377386, 9.998486224644262)
(0.44082810336479544, 10.99757795943082)
(0.4566592515880744, 11.996669694217378)
(0.47042050348896813, 12.995761429003934)
(0.48289854168278884, 13.994853163790493)
(0.4972688512457014, 14.993944898577052)
(0.5098607797978458, 15.993036633363609)
(0.5194086186317814, 16.992128368150166)
(0.5292165956933478, 17.991220102936726)
(0.5397513489412111, 18.99031183772328)
(0.5495374645008233, 19.98940357250984)
(0.5585755738924363, 20.988495307296397)
(0.569750381525454, 21.987587042082954)
(0.5788276890547444, 22.986678776869514)
(0.5889246594981864, 23.98577051165607)
(0.59776501675872, 24.984862246442628)
(0.6067302666100951, 25.983953981229185)
(0.6143269625027951, 26.98304571601574)
(0.6212849988025461, 27.982137450802302)
(0.6288552185079805, 28.98122918558886)
(0.6362316417533519, 29.980320920375412)
(0.6453280038233917, 30.979412655161976)
(0.6522782401204505, 31.97850438994853)
(0.6605891395914751, 32.977596124735086)
(0.6691189439951611, 33.97668785952165)
(0.6760988061782441, 34.97577959430821)
(0.6843286517831917, 35.97487132909476)
(0.6906613946818768, 36.97396306388132)
(0.6974866505689972, 37.973054798667874)
(0.7030349512308272, 38.972146533454435)
(0.7091787931892044, 39.971238268240995)
(0.7165417962007284, 40.97033000302755)
(0.7236120897380252, 41.96942173781411)
(0.7303858805656228, 42.96851347260067)
(0.7376477467352278, 43.96760520738722)
(0.7442416984962476, 44.96669694217378)
(0.7510462634558496, 45.96578867696034)
(0.7579379131319818, 46.9648804117469)
(0.7659908827271037, 47.96397214653346)
(0.7732501971189298, 48.96306388132001)
(0.7805613393125629, 49.96215561610657)
(0.7879571911607608, 50.961247350893125)
(0.796117022146819, 51.960339085679685)
(0.8016487856319184, 52.959430820466245)
(0.8070622579668044, 53.9585225552528)
(0.8150974520792839, 54.95761429003936)
(0.8226797454331872, 55.95670602482592)
(0.8299591621365784, 56.95579775961247)
(0.8373297596088489, 57.95488949439903)
(0.8479478390669437, 58.953981229185594)
(0.8589529283083992, 59.95307296397214)
(0.8674345742239603, 60.95216469875871)
(0.8752257466069254, 61.95125643354527)
(0.8825230294614749, 62.950348168331814)
(0.8905888977050573, 63.949439903118375)
(0.8993504571480019, 64.94853163790494)
(0.9083499176444713, 65.94762337269148)
(0.9185625230069244, 66.94671510747806)
(0.9281898412514336, 67.94580684226462)
(0.9380433595188664, 68.94489857705116)
(0.9477097244287913, 69.94399031183772)
(0.9585831805604785, 70.94308204662428)
(0.9685274222668637, 71.94217378141083)
(0.9799950082080487, 72.94126551619739)
(0.9901915607197342, 73.94035725098395)
(0.9997810702457492, 74.93944898577051)
(1.009215652214925, 75.93854072055707)
(1.0202910502360365, 76.93763245534363)
(1.0310227911581724, 77.93672419013018)
(1.0434085588304465, 78.93581592491674)
(1.05553667789186, 79.9349076597033)
(1.066219115509836, 80.93399939448986)
(1.077364971179534, 81.93309112927642)
(1.0890131462789991, 82.93218286406298)
(1.1032716164823893, 83.93127459884953)
(1.1162783820705542, 84.93036633363609)
(1.1282025599445562, 85.92945806842265)
(1.1428297464532604, 86.9285498032092)
(1.1575431471437574, 87.92764153799575)
(1.171432070045381, 88.92673327278231)
(1.1860680216302795, 89.92582500756887)
(1.2029892691632815, 90.92491674235544)
(1.2233141490258996, 91.924008477142)
(1.2456852492368784, 92.92310021192854)
(1.2720535906454127, 93.9221919467151)
(1.303868360019315, 94.92128368150166)
(1.3415747663059903, 95.92037541628822)
(1.3868940127170981, 96.91946715107478)
(1.4383558315183698, 97.91855888586134)
(1.5199330610702564, 98.9176506206479)
(1.765594595029234, 99.91674235543445)
};
\addplot[solid, blue, thick, mark=none] coordinates{
(0.25746168749133397, 0.007568876778686043)
(0.26509954775991834, 1.006660611565244)
(0.2665689922433437, 2.005752346351801)
(0.26734285363814053, 3.004844081138359)
(0.2679002019164998, 4.003935815924916)
(0.2683051990187068, 5.003027550711474)
(0.26868707472720915, 6.002119285498033)
(0.2689291838347194, 7.00121102028459)
(0.2691646087497785, 8.000302755071148)
(0.2693902199861751, 8.999394489857705)
(0.2696862286979267, 9.998486224644262)
(0.2698308905418772, 10.99757795943082)
(0.269970218693476, 11.996669694217378)
(0.2701048287261656, 12.995761429003934)
(0.27027805093513846, 13.994853163790493)
(0.2704389095250881, 14.993944898577052)
(0.2705952212265284, 15.993036633363609)
(0.270804840509674, 16.992128368150166)
(0.271088072219248, 17.991220102936726)
(0.2713306258805302, 18.99031183772328)
(0.27160846525146554, 19.98940357250984)
(0.27189340347251095, 20.988495307296397)
(0.272248993227469, 21.987587042082954)
(0.27250701410359846, 22.986678776869514)
(0.2728390178004208, 23.98577051165607)
(0.27320798345222125, 24.984862246442628)
(0.2735630290945522, 25.983953981229185)
(0.27395600448656143, 26.98304571601574)
(0.27454494736176743, 27.982137450802302)
(0.276439818282768, 28.98122918558886)
(0.28694684840327345, 29.980320920375412)
(0.2986185520339744, 30.979412655161976)
(0.31169389603023984, 31.97850438994853)
(0.32813858927841927, 32.977596124735086)
(0.34410805000906686, 33.97668785952165)
(0.3590538795046547, 34.97577959430821)
(0.37501325514473643, 35.97487132909476)
(0.3896660095433637, 36.97396306388132)
(0.4057088712421409, 37.973054798667874)
(0.42138564732745, 38.972146533454435)
(0.4380632617485289, 39.971238268240995)
(0.4532115848671468, 40.97033000302755)
(0.469352377282936, 41.96942173781411)
(0.4873834838238608, 42.96851347260067)
(0.5039439979683824, 43.96760520738722)
(0.5198173241112131, 44.96669694217378)
(0.5332537007932019, 45.96578867696034)
(0.546488751578737, 46.9648804117469)
(0.5606997678401475, 47.96397214653346)
(0.5763201432636109, 48.96306388132001)
(0.5897896613156197, 49.96215561610657)
(0.6039110852687709, 50.961247350893125)
(0.6177038339146237, 51.960339085679685)
(0.63162580608985, 52.959430820466245)
(0.6439203361362538, 53.9585225552528)
(0.6574014012188845, 54.95761429003936)
(0.6698702143363571, 55.95670602482592)
(0.6818774317263291, 56.95579775961247)
(0.692149089968257, 57.95488949439903)
(0.7016652976201017, 58.953981229185594)
(0.7103913944158075, 59.95307296397214)
(0.7196462847466807, 60.95216469875871)
(0.7324740346813264, 61.95125643354527)
(0.7437369307231945, 62.950348168331814)
(0.7558690893115501, 63.949439903118375)
(0.7681216217786423, 64.94853163790494)
(0.7803473617293868, 65.94762337269148)
(0.7945422991016295, 66.94671510747806)
(0.808607814028635, 67.94580684226462)
(0.822579093907743, 68.94489857705116)
(0.8359237195655357, 69.94399031183772)
(0.8486680124094899, 70.94308204662428)
(0.8618082402322886, 71.94217378141083)
(0.8745185120397095, 72.94126551619739)
(0.8881097066915286, 73.94035725098395)
(0.9022221674148513, 74.93944898577051)
(0.9157312989592936, 75.93854072055707)
(0.9279688538254733, 76.93763245534363)
(0.9408116013417619, 77.93672419013018)
(0.9553826268268659, 78.93581592491674)
(0.9692105716863969, 79.9349076597033)
(0.9831891896884706, 80.93399939448986)
(0.997697764070792, 81.93309112927642)
(1.0112291975635845, 82.93218286406298)
(1.0277696647381616, 83.93127459884953)
(1.0443439044715863, 84.93036633363609)
(1.0584872742299176, 85.92945806842265)
(1.0768906269685135, 86.9285498032092)
(1.0917943654428668, 87.92764153799575)
(1.1092464416822967, 88.92673327278231)
(1.125745533276977, 89.92582500756887)
(1.1400013850001742, 90.92491674235544)
(1.1538788726857505, 91.924008477142)
(1.1746787278655983, 92.92310021192854)
(1.2017564486289447, 93.9221919467151)
(1.2327857137007674, 94.92128368150166)
(1.2766833130506414, 95.92037541628822)
(1.3217392045892484, 96.91946715107478)
(1.3850633590099086, 97.91855888586134)
(1.4734887552894476, 98.9176506206479)
(1.7569486509129963, 99.91674235543445)
};
\addplot[solid, red, thick, mark=none] coordinates{
(0.2592130144755187, 0.007568876778686043)
(0.265688383614129, 1.006660611565244)
(0.2670225813307146, 2.005752346351801)
(0.2677238273931536, 3.004844081138359)
(0.2682733579076533, 4.003935815924916)
(0.2686870747272092, 5.003027550711474)
(0.2689535351062295, 6.002119285498033)
(0.2691914599221523, 7.00121102028459)
(0.26935968358819967, 8.000302755071148)
(0.26960005306575097, 8.999394489857705)
(0.2697688222182829, 9.998486224644262)
(0.2698601870313802, 10.99757795943082)
(0.269970218693476, 11.996669694217378)
(0.2700828960958333, 12.995761429003934)
(0.27020893249428063, 13.994853163790493)
(0.2703347722783323, 14.993944898577052)
(0.27044269698391843, 15.993036633363609)
(0.27055455982561477, 16.992128368150166)
(0.2707204164782034, 17.991220102936726)
(0.270906294729738, 18.99031183772328)
(0.2710619878839822, 19.98940357250984)
(0.27130603621396243, 20.988495307296397)
(0.2715505258679191, 21.987587042082954)
(0.27183831916352524, 22.986678776869514)
(0.2724988102900374, 23.98577051165607)
(0.2741123789128432, 24.984862246442628)
(0.2800823048043721, 25.983953981229185)
(0.28809438271044535, 26.98304571601574)
(0.2967116730201748, 27.982137450802302)
(0.30682002188015206, 28.98122918558886)
(0.3198610675807051, 29.980320920375412)
(0.3320915890166645, 30.979412655161976)
(0.3445837286915773, 31.97850438994853)
(0.3577620000676635, 32.977596124735086)
(0.3718960580524425, 33.97668785952165)
(0.3860389517809995, 34.97577959430821)
(0.40017368681887655, 35.97487132909476)
(0.4131799123825897, 36.97396306388132)
(0.42747280090301376, 37.973054798667874)
(0.44186898570028404, 38.972146533454435)
(0.4590536815683698, 39.971238268240995)
(0.4747536890909256, 40.97033000302755)
(0.4898349909674685, 41.96942173781411)
(0.5070744304037225, 42.96851347260067)
(0.5226147841671578, 43.96760520738722)
(0.5364393170319907, 44.96669694217378)
(0.5515641464932607, 45.96578867696034)
(0.5643377759393801, 46.9648804117469)
(0.5804505840870535, 47.96397214653346)
(0.5940688163035351, 48.96306388132001)
(0.6075384692066309, 49.96215561610657)
(0.6189319965208018, 50.961247350893125)
(0.6336383723753949, 51.960339085679685)
(0.6475537559206515, 52.959430820466245)
(0.6601530223325845, 53.9585225552528)
(0.6723193737586289, 54.95761429003936)
(0.6823267067506927, 55.95670602482592)
(0.6925778688769391, 56.95579775961247)
(0.7012104297567636, 57.95488949439903)
(0.7087798749000674, 58.953981229185594)
(0.7162106277034533, 59.95307296397214)
(0.7273645894887659, 60.95216469875871)
(0.7395804921281683, 61.95125643354527)
(0.7507981786368629, 62.950348168331814)
(0.7653867723554337, 63.949439903118375)
(0.7795265697991394, 64.94853163790494)
(0.7933375338503887, 65.94762337269148)
(0.8080805160590295, 66.94671510747806)
(0.8220761052176009, 67.94580684226462)
(0.8363086656413155, 68.94489857705116)
(0.8510262158801135, 69.94399031183772)
(0.864324194369184, 70.94308204662428)
(0.8773169114086944, 71.94217378141083)
(0.8895567328045711, 72.94126551619739)
(0.904776269623676, 73.94035725098395)
(0.9184857176627409, 74.93944898577051)
(0.930001225324037, 75.93854072055707)
(0.9419364509275079, 76.93763245534363)
(0.9550038764245791, 77.93672419013018)
(0.969560970203122, 78.93581592491674)
(0.9828786738985335, 79.9349076597033)
(0.9964815894161694, 80.93399939448986)
(1.0092886326212946, 81.93309112927642)
(1.0234024067962482, 82.93218286406298)
(1.0385953611435554, 83.93127459884953)
(1.0552772844078997, 84.93036633363609)
(1.0712646190355541, 85.92945806842265)
(1.0874420111188297, 86.9285498032092)
(1.1019661691787122, 87.92764153799575)
(1.1184342084257808, 88.92673327278231)
(1.1315689581868347, 89.92582500756887)
(1.1453532619654394, 90.92491674235544)
(1.1638060293332477, 91.924008477142)
(1.185487961715699, 92.92310021192854)
(1.214140375873689, 93.9221919467151)
(1.2444230896726045, 94.92128368150166)
(1.2830323681832307, 95.92037541628822)
(1.3298955327699433, 96.91946715107478)
(1.3870265310144474, 97.91855888586134)
(1.4719337144751496, 98.9176506206479)
(1.7565128515100734, 99.91674235543445)
};
\addplot[solid, magenta, thick, mark=none] coordinates{
(-0.11833990302894268, 0.030275507114744173)
(0.10385846815580707, 1.0293672419013018)
(0.13163589733397094, 2.0284589766878596)
(0.15753238376426043, 3.0275507114744173)
(0.1831974821166531, 4.026642446260976)
(0.2042732628591773, 5.0257341810475324)
(0.22384909889909296, 6.02482591583409)
(0.23922899115678384, 7.023917650620648)
(0.25624571540514923, 8.023009385407205)
(0.2734444263389859, 9.022101120193764)
(0.2867127224109619, 10.02119285498032)
(0.3049700153143631, 11.020284589766877)
(0.32182222625448437, 12.019376324553436)
(0.3367034617203354, 13.018468059339995)
(0.34656531859362955, 14.017559794126552)
(0.3643142306665359, 15.016651528913108)
(0.3758688756522449, 16.015743263699665)
(0.3863616785876473, 17.014834998486226)
(0.3973840043339758, 18.013926733272783)
(0.4084428087720275, 19.01301846805934)
(0.41666118517387263, 20.012110202845896)
(0.42953273743081477, 21.011201937632457)
(0.4401748373012293, 22.010293672419014)
(0.45128099377035186, 23.00938540720557)
(0.46219335125188443, 24.00847714199213)
(0.4750440447950875, 25.007568876778684)
(0.48302040963246556, 26.00666061156524)
(0.4911992054304503, 27.0057523463518)
(0.502151119026529, 28.00484408113836)
(0.5092619877217097, 29.00393581592492)
(0.5159334418815862, 30.003027550711476)
(0.5228257750121565, 31.002119285498033)
(0.5288503624963478, 32.00121102028459)
(0.5352625002294111, 33.00030275507115)
(0.542279341463041, 33.99939448985771)
(0.5493952805341613, 34.99848622464427)
(0.5546855751109452, 35.99757795943082)
(0.5623048642564468, 36.996669694217374)
(0.5700868866754735, 37.995761429003934)
(0.5753537308222385, 38.994853163790495)
(0.5808866973986532, 39.99394489857705)
(0.5858360911581908, 40.99303663336361)
(0.5907475407773211, 41.99212836815017)
(0.5943517152983994, 42.99122010293672)
(0.6011468306578901, 43.99031183772328)
(0.6048230197884578, 44.989403572509836)
(0.6086123223358103, 45.9884953072964)
(0.6146990659697165, 46.98758704208296)
(0.6199014607159279, 47.98667877686951)
(0.6234930567539532, 48.98577051165607)
(0.6277344176446594, 49.98486224644263)
(0.6321264478233386, 50.98395398122919)
(0.6358924353994103, 51.98304571601574)
(0.6412332864425783, 52.982137450802306)
(0.6446957703384761, 53.981229185588866)
(0.6501356830554145, 54.98032092037541)
(0.65568707825772, 55.97941265516197)
(0.6612318815670238, 56.97850438994854)
(0.669340580652459, 57.977596124735086)
(0.6786179506716268, 58.97668785952165)
(0.689397992079206, 59.97577959430821)
(0.7005967235952899, 60.97487132909476)
(0.7110292194705159, 61.97396306388132)
(0.7216316756223426, 62.97305479866788)
(0.7297962093635159, 63.972146533454435)
(0.7385866383161078, 64.971238268241)
(0.7477378893220465, 65.97033000302756)
(0.7609075279403873, 66.9694217378141)
(0.7746228175930252, 67.96851347260066)
(0.7870026257177258, 68.96760520738722)
(0.7958188359881645, 69.96669694217378)
(0.8066500005341279, 70.96578867696034)
(0.8178296870448337, 71.9648804117469)
(0.8300652512432461, 72.96397214653345)
(0.8403580594502521, 73.96306388132001)
(0.8526122423007044, 74.96215561610657)
(0.8625714912643057, 75.96124735089312)
(0.8715179812639604, 76.96033908567969)
(0.8824253277551346, 77.95943082046625)
(0.8916126133678965, 78.9585225552528)
(0.9064348635897634, 79.95761429003936)
(0.9206843663478171, 80.95670602482592)
(0.9311673420359402, 81.95579775961247)
(0.943501343734851, 82.95488949439903)
(0.9577875952960105, 83.95398122918559)
(0.9724741320969512, 84.95307296397215)
(0.9850580586687774, 85.95216469875871)
(0.9964718062836837, 86.95125643354527)
(1.0082650307866492, 87.95034816833181)
(1.018444851730612, 88.94943990311837)
(1.0287448572373072, 89.94853163790494)
(1.037327054905245, 90.94762337269148)
(1.0545589037440406, 91.94671510747806)
(1.0712610111386007, 92.94580684226462)
(1.092317105414452, 93.94489857705116)
(1.1194878860384265, 94.94399031183772)
(1.1590176023780414, 95.94308204662428)
(1.2145399075585352, 96.94217378141083)
(1.277265051149417, 97.94126551619739)
(1.3814877461950787, 98.94035725098395)
(1.740073495038477, 99.93944898577051)
};

==> figures/raw_data/abr_synth/buff_time.tex <==
\addplot[solid, green!70!black, thick, mark=none] coordinates{
(0, 0.0)
(1, 0.9813602892074523)
(2, 3.1204563996782415)
(3, 4.6246044899235805)
(4, 5.36865308885263)
(5, 5.150011229506945)
(6, 5.08686668559439)
(7, 4.721259328012323)
(8, 4.464620554641828)
(9, 4.271574171650486)
(10, 4.582888347396116)
(11, 4.67608077064601)
(12, 4.513857109712304)
(13, 4.590095592293089)
(14, 4.708274681957765)
(15, 4.703039281372365)
(16, 5.013509660258199)
(17, 5.163600499907091)
(18, 4.895055289234546)
(19, 4.927941533380567)
(20, 5.088010349410357)
(21, 4.925054679187366)
(22, 4.950313705467059)
(23, 5.014126598089371)
(24, 5.180585708770876)
(25, 5.1029882561960065)
(26, 4.90478350430081)
(27, 5.076178478524209)
(28, 5.818606799930475)
(29, 5.385033613958036)
(30, 5.07512789105135)
(31, 5.088363387580891)
(32, 5.048318641947165)
(33, 5.216952646089055)
(34, 5.1191370452021205)
};
\addplot[solid, blue, thick, mark=none] coordinates{
(0, 0.0)
(1, 0.0)
(2, 7.11662896149072)
(3, 9.628679365347537)
(4, 11.276347795472821)
(5, 11.083021787741625)
(6, 10.65654344458697)
(7, 10.447523125661755)
(8, 9.636364328912189)
(9, 9.853837939760442)
(10, 10.518230177594429)
(11, 10.438760548856264)
(12, 9.965841797321936)
(13, 10.525102318387844)
(14, 10.139595420854503)
(15, 10.401822248287786)
(16, 10.909140298489408)
(17, 10.956065663653334)
(18, 10.623858746803633)
(19, 10.628650343440109)
(20, 10.79945605488578)
(21, 10.6210336430105)
(22, 10.680992749620913)
(23, 10.518413428543584)
(24, 10.660370294620657)
(25, 11.038527481626648)
(26, 10.545213973319164)
(27, 10.241535573902404)
(28, 11.079209109069781)
(29, 10.822196757309927)
(30, 10.616030108986546)
(31, 10.902343753796364)
(32, 10.634913594872696)
(33, 10.74428509030144)
(34, 10.544390129470619)
};
\addplot[solid, red, thick, mark=none] coordinates{
(0, 0.0)
(1, 2.425630518392992)
(2, 8.79107784774554)
(3, 10.853966621391109)
(4, 12.07528015164041)
(5, 11.494744496433693)
(6, 10.75313095195401)
(7, 10.379708860909254)
(8, 9.531278192059908)
(9, 9.571253077671459)
(10, 10.259659448861157)
(11, 10.159386043977724)
(12, 9.734887849429805)
(13, 10.01536345557544)
(14, 9.813286028484166)
(15, 9.983088081409527)
(16, 10.56172318494327)
(17, 10.36136981438239)
(18, 10.126792532537458)
(19, 10.14745931308889)
(20, 10.360449452219338)
(21, 10.11819388717538)
(22, 10.085763760989874)
(23, 10.119550625098489)
(24, 10.401008444610525)
(25, 10.540685346303224)
(26, 10.08683327920095)
(27, 10.010888285464775)
(28, 10.4980657707556)
(29, 10.281517711716054)
(30, 10.231169020202223)
(31, 10.356748845646566)
(32, 10.090626104051847)
(33, 10.42046944252931)
(34, 10.143818047451283)
};


==> figures/raw_data/abr_synth/buffer_mse_cdf.tex <==
\addplot[solid, green!70!black, thick, mark=none] coordinates{
(0.0036184025493355876, 1.3888888888888888)
(0.004878650180010029, 2.7777777777777777)
(0.006081665954865524, 4.166666666666666)
(0.006363487836036971, 5.555555555555555)
(0.008302078427949316, 6.944444444444445)
(0.014511366367924923, 8.333333333333332)
(0.014749124291235859, 9.722222222222223)
(0.01671191987818499, 11.11111111111111)
(0.01851535053297369, 12.5)
(0.018883430641679657, 13.88888888888889)
(0.01895992431964091, 15.277777777777779)
(0.024271746773848173, 16.666666666666664)
(0.0254173315490261, 18.055555555555554)
(0.03611156578720162, 19.444444444444446)
(0.044687065764955174, 20.833333333333336)
(0.05504691538149484, 22.22222222222222)
(0.07853750386732906, 23.61111111111111)
(0.10040667568243287, 25.0)
(0.1141264622153819, 26.38888888888889)
(0.11945458502121181, 27.77777777777778)
(0.16847548338651183, 29.166666666666668)
(0.19135640659466008, 30.555555555555557)
(0.19368652837040126, 31.944444444444443)
(0.22513888512615263, 33.33333333333333)
(0.2319229644572196, 34.72222222222222)
(0.24229777424660512, 36.11111111111111)
(0.2691480918773445, 37.5)
(0.2704684635497656, 38.88888888888889)
(0.2775469439167777, 40.27777777777778)
(0.29134363282297054, 41.66666666666667)
(0.3067120871697715, 43.05555555555556)
(0.3307145933941183, 44.44444444444444)
(0.3537060770654004, 45.83333333333333)
(0.389473857667305, 47.22222222222222)
(0.40264219948043395, 48.61111111111111)
(0.42052301971651307, 50.0)
(0.4221319695479469, 51.388888888888886)
(0.4503904298625836, 52.77777777777778)
(0.46569179331817045, 54.166666666666664)
(0.499761860593346, 55.55555555555556)
(0.5321477665742599, 56.94444444444444)
(0.5426394860622095, 58.333333333333336)
(0.5549882275618241, 59.72222222222222)
(0.5608869572043267, 61.111111111111114)
(0.5617189316163773, 62.5)
(0.5659397668897663, 63.888888888888886)
(0.575607435241993, 65.27777777777779)
(0.5921053172738262, 66.66666666666666)
(0.5923239944110187, 68.05555555555556)
(0.6194364252109416, 69.44444444444444)
(0.6366155719727118, 70.83333333333334)
(0.6684026793799728, 72.22222222222221)
(0.6810292728565116, 73.61111111111111)
(0.7249253391198205, 75.0)
(0.7588123086671535, 76.38888888888889)
(0.8554880870377373, 77.77777777777779)
(0.8580875914258972, 79.16666666666666)
(0.8898618121761832, 80.55555555555556)
(1.0107191481712936, 81.94444444444444)
(1.0292216288993035, 83.33333333333334)
(1.1417344878701452, 84.72222222222221)
(1.4909436639093774, 86.11111111111111)
(1.5144304267940643, 87.5)
(1.5505714856010113, 88.88888888888889)
(2.000565572766798, 90.27777777777779)
(2.0481702774938317, 91.66666666666666)
(2.159836484860094, 93.05555555555556)
(2.2446082642717, 94.44444444444444)
(2.4051812312486174, 95.83333333333334)
(2.7994420232483725, 97.22222222222221)
(2.8429992376769344, 98.61111111111111)
(3.4877823178123775, 100.0)
};
\addplot[solid, blue, thick, mark=none] coordinates{
(0.0027569427403395692, 1.3888888888888888)
(0.007495125808720343, 2.7777777777777777)
(0.009956970373934313, 4.166666666666666)
(0.029946626685448157, 5.555555555555555)
(0.031445003391698145, 6.944444444444445)
(0.03200830570755017, 8.333333333333332)
(0.034639519931745986, 9.722222222222223)
(0.04665908674554423, 11.11111111111111)
(0.0816961315917127, 12.5)
(0.10558828439175207, 13.88888888888889)
(0.1071986242637794, 15.277777777777779)
(0.14624079549797606, 16.666666666666664)
(0.29661984044775563, 18.055555555555554)
(0.40889559272329395, 19.444444444444446)
(0.40899341909794235, 20.833333333333336)
(0.4262250475386471, 22.22222222222222)
(0.43084505117475624, 23.61111111111111)
(0.46971548356643206, 25.0)
(0.47296577433498926, 26.38888888888889)
(0.5842473817639838, 27.77777777777778)
(0.6224321737687842, 29.166666666666668)
(0.6366905661401255, 30.555555555555557)
(0.6721454255644985, 31.944444444444443)
(0.6936895016174591, 33.33333333333333)
(0.7218849590734306, 34.72222222222222)
(0.7787304947550853, 36.11111111111111)
(0.8361067602709508, 37.5)
(0.8379438923032441, 38.88888888888889)
(0.8434298197798767, 40.27777777777778)
(0.8558958301151897, 41.66666666666667)
(0.9469857442648538, 43.05555555555556)
(0.9934227360284771, 44.44444444444444)
(1.0317454916011488, 45.83333333333333)
(1.0387601833197821, 47.22222222222222)
(1.1474214151698823, 48.61111111111111)
(1.211692752501191, 50.0)
(1.2555892663357193, 51.388888888888886)
(1.2614980564396596, 52.77777777777778)
(1.2813589258006484, 54.166666666666664)
(1.3838656637475093, 55.55555555555556)
(1.4579531471342684, 56.94444444444444)
(1.5272375157416433, 58.333333333333336)
(1.5956179679930158, 59.72222222222222)
(1.5968711747792794, 61.111111111111114)
(1.844580398672206, 62.5)
(2.077984859972958, 63.888888888888886)
(2.1151816492121087, 65.27777777777779)
(2.1414171183802586, 66.66666666666666)
(2.3259319860888024, 68.05555555555556)
(2.3844675227698797, 69.44444444444444)
(2.5010651549214202, 70.83333333333334)
(2.5609764051947574, 72.22222222222221)
(2.5951511177222244, 73.61111111111111)
(2.727598604311462, 75.0)
(2.7611560238636743, 76.38888888888889)
(2.80832808847164, 77.77777777777779)
(2.8739472573024845, 79.16666666666666)
(2.908945135700819, 80.55555555555556)
(3.0081796087505195, 81.94444444444444)
(3.172670152151618, 83.33333333333334)
(3.4431383307822703, 84.72222222222221)
(3.782540721706961, 86.11111111111111)
(3.892024814387612, 87.5)
(4.40226923889373, 88.88888888888889)
(5.038821556154869, 90.27777777777779)
(6.507659759839981, 91.66666666666666)
(7.029167436952682, 93.05555555555556)
(7.343369509613378, 94.44444444444444)
(8.171700773628361, 95.83333333333334)
(19.81222972544621, 97.22222222222221)
(20.080085797578594, 98.61111111111111)
(22.74815260933635, 100.0)
};
\addplot[solid, red, thick, mark=none] table {%
0.0318857477074741 0
0.0364962335023818 1.5625
0.0535572733438283 3.125
0.0898186343498467 4.6875
0.0940198987657325 6.25
0.111468833669154 7.8125
0.419881963505556 9.375
0.474393595698074 10.9375
0.487401384707652 12.5
0.491703192073224 14.0625
0.494646930576592 15.625
0.623920761963056 17.1875
0.633743121577011 18.75
0.700401540785354 20.3125
0.708228151673986 21.875
0.726179463053364 23.4375
0.735643990379735 25
0.745101079329847 26.5625
0.829527875864125 28.125
0.831263856423002 29.6875
0.871499454037442 31.25
0.884997944713269 32.8125
0.888789227853594 34.375
0.936583981622246 35.9375
0.973375691473427 37.5
1.00316388918506 39.0625
1.0437977591356 40.625
1.04906036875599 42.1875
1.07779733950411 43.75
1.13398090960767 45.3125
1.1965717564139 46.875
1.2581299951736 48.4375
1.26767923118145 50
1.3150960940065 51.5625
1.31674504978872 53.125
1.46298746686746 54.6875
1.4963624633464 56.25
1.73312378542068 57.8125
1.81489949248752 59.375
1.98246501620122 60.9375
2.05267659648799 62.5
2.14082117835699 64.0625
2.41175150234669 65.625
2.43765682414252 67.1875
2.56530257209728 68.75
2.61786523512528 70.3125
2.61803963355653 71.875
2.66059946146576 73.4375
2.82548182199261 75
2.84257066823686 76.5625
2.90684309973996 78.125
2.96536675322401 79.6875
2.98211047843471 81.25
3.1155848210996 82.8125
3.31686484629755 84.375
3.60755403656733 85.9375
4.07635100845302 87.5
4.12811412690277 89.0625
4.32222424007726 90.625
4.36663648461467 92.1875
5.37897724297531 93.75
19.1487492384046 95.3125
19.7623869888785 96.875
21.5437405019093 98.4375
};


==> figures/raw_data/load_balancing/latency_mape.tex <==
\addplot[solid, green!70!black, thick, mark=none] table {%
18.4502781801223 0
18.5195418225765 1.78571428571429
18.5881893914436 3.57142857142857
18.6134272828567 5.35714285714286
18.6650560301591 7.14285714285714
18.9453628609138 8.92857142857143
18.9587643913725 10.7142857142857
18.9731688879539 12.5
19.0827543213717 14.2857142857143
19.3324861595118 16.0714285714286
19.4185878485702 17.8571428571429
19.4899161632357 19.6428571428571
19.5728044567471 21.4285714285714
19.899893709852 23.2142857142857
24.827982798245 25
24.9970870526 26.7857142857143
25.0656091222561 28.5714285714286
25.1071632955337 30.3571428571429
25.2882396422434 32.1428571428571
25.5225957243934 33.9285714285714
25.6599195785169 35.7142857142857
25.7028704201442 37.5
26.4140504956228 39.2857142857143
26.5159825492234 41.0714285714286
26.5445833600001 42.8571428571429
26.7228041554858 44.6428571428571
26.744140280315 46.4285714285714
26.8880513417985 48.2142857142857
26.9733037680742 50
27.2479836707572 51.7857142857143
27.450552219405 53.5714285714286
27.5186760566285 55.3571428571429
27.5225520067066 57.1428571428571
27.5510626065641 58.9285714285714
27.832230953371 60.7142857142857
30.6473396820535 62.5
31.2585440738824 64.2857142857143
31.3675086233941 66.0714285714286
31.9778519317761 67.8571428571429
32.2307022703296 69.6428571428571
32.8683099809999 71.4285714285714
32.8754625519921 73.2142857142857
33.1151965725051 75
35.4193469887701 76.7857142857143
38.1991011497111 78.5714285714286
38.6392518521021 80.3571428571429
39.6940389637663 82.1428571428571
41.1402169588758 83.9285714285714
42.2207347191105 85.7142857142857
43.6497857550536 87.5
43.7390808203081 89.2857142857143
43.9999119334245 91.0714285714286
45.7586416079666 92.8571428571429
46.1616149817564 94.6428571428571
46.3169250915744 96.4285714285714
46.7472350158313 98.2142857142857
};
\addplot[solid, red, thick, mark=none] 
table {%
32.9239403317749 0
33.6250184092309 0.833333333333333
35.2650721883496 1.66666666666667
37.4971791903499 2.5
39.2365564992343 3.33333333333333
41.622348289224 4.16666666666667
45.9936382059362 5
48.419785328681 5.83333333333333
49.151232651489 6.66666666666667
49.1702921711054 7.5
49.834272152395 8.33333333333333
53.8654383341236 9.16666666666667
55.4184663674639 10
58.9896698783296 10.8333333333333
61.9106691043075 11.6666666666667
63.1404723780777 12.5
64.7585728032125 13.3333333333333
65.1040956871009 14.1666666666667
66.064810497652 15
67.6080726160199 15.8333333333333
67.7823385082395 16.6666666666667
67.994460619492 17.5
70.3078924593488 18.3333333333333
71.5771355359933 19.1666666666667
75.6282046554794 20
79.1370732182242 20.8333333333333
85.8612777859108 21.6666666666667
91.2124253515959 22.5
108.578916527637 23.3333333333333
132.931091104555 24.1666666666667
139.883809311387 25
158.034355467916 25.8333333333333
169.455059681492 26.6666666666667
170.030692390702 27.5
172.919590381882 28.3333333333333
175.339619761209 29.1666666666667
176.317127407875 30
196.596448440932 30.8333333333333
201.41113411399 31.6666666666667
209.902880774839 32.5
212.431923813614 33.3333333333333
214.992170827789 34.1666666666667
216.21145271588 35
220.046101170874 35.8333333333333
238.172202717237 36.6666666666667
241.324321932541 37.5
245.628934827886 38.3333333333333
254.309164680323 39.1666666666667
287.030629003919 40
292.755234474258 40.8333333333333
303.605024850659 41.6666666666667
306.45822840657 42.5
314.103482623683 43.3333333333333
324.638807600155 44.1666666666667
337.340899863762 45
338.21895041393 45.8333333333333
363.457023917233 46.6666666666667
387.12322442435 47.5
459.99802950636 48.3333333333333
464.823705694569 49.1666666666667
470.781691260449 50
483.374620377754 50.8333333333333
489.702253272915 51.6666666666667
512.435151977496 52.5
564.073471240224 53.3333333333333
614.970196081455 54.1666666666667
642.382602003031 55
644.872760347039 55.8333333333333
687.898760718543 56.6666666666667
700.066710262664 57.5
760.288353110703 58.3333333333333
762.064312019204 59.1666666666667
771.496982822743 60
778.330582111545 60.8333333333333
786.462687015623 61.6666666666667
807.747194068489 62.5
882.042833058872 63.3333333333333
904.34790343975 64.1666666666667
915.681148679231 65
1163.77065331838 65.8333333333333
1319.34692268066 66.6666666666667
1374.8299985624 67.5
1457.78657703606 68.3333333333333
1511.63614646318 69.1666666666667
1536.86848573434 70
1662.67270310564 70.8333333333333
1686.53408314854 71.6666666666667
1723.16055164162 72.5
1790.68157407585 73.3333333333333
1797.46238017744 74.1666666666667
1799.79684091723 75
1820.95263227529 75.8333333333333
1953.18409277126 76.6666666666667
2117.18510122238 77.5
2172.89042989622 78.3333333333333
2214.89506669715 79.1666666666667
2261.16754921454 80
2312.04289028391 80.8333333333333
2529.41685271657 81.6666666666667
2736.26417120156 82.5
2747.13330076364 83.3333333333333
2877.12659373882 84.1666666666667
3028.37156692723 85
3523.20885081886 85.8333333333333
4306.08862447219 86.6666666666667
5881.26173836961 87.5
6658.41923113481 88.3333333333333
7159.58611007854 89.1666666666667
7268.0707254623 90
7527.38156045399 90.8333333333333
8319.76139321422 91.6666666666667
8523.7720028268 92.5
8629.37638694084 93.3333333333333
8808.02579912729 94.1666666666667
9536.20361630988 95
9548.78985493099 95.8333333333333
9726.13297365872 96.6666666666667
9808.95233206269 97.5
11479.1623198591 98.3333333333333
16014.0658233836 99.1666666666667
};


==> figures/raw_data/load_balancing/latency_pol.tex <==
\addplot [thick, green!70!black]
table {%
-6.02319570954097 0
8.48185491008849 3.2258064516129
12.7317613113516 6.45161290322581
16.8801476008951 9.67741935483871
20.5275917963623 12.9032258064516
24.1619749525363 16.1290322580645
28.4019117233077 19.3548387096774
33.4355795330979 22.5806451612903
39.0338986153317 25.8064516129032
45.1267970340692 29.0322580645161
51.9445339695744 32.258064516129
59.35450403661 35.4838709677419
67.6353711722913 38.7096774193548
76.6919017415433 41.9354838709677
86.8393045286575 45.1612903225806
98.1493755631414 48.3870967741936
110.962969468617 51.6129032258064
126.631487398746 54.8387096774194
145.420258591479 58.0645161290323
167.434956035928 61.2903225806452
192.138307493101 64.5161290322581
222.386579286796 67.741935483871
261.083268816416 70.9677419354839
313.680174747333 74.1935483870968
383.272159501551 77.4193548387097
484.136278893656 80.6451612903226
650.186334864652 83.8709677419355
963.582526862551 87.0967741935484
1720.10979005838 90.3225806451613
3925.97651181694 93.5483870967742
22277.2757078501 96.7741935483871
};
\addplot [thick, red, solid]
table {%
2.11116951586348 0
11.1347924954852 3.2258064516129
15.6925361415175 6.45161290322581
20.6654640214955 9.67741935483871
26.2254164375181 12.9032258064516
32.2390743411915 16.1290322580645
39.4691431164943 19.3548387096774
46.2660600790942 22.5806451612903
54.8083893284945 25.8064516129032
64.1414753858515 29.0322580645161
76.0252339057811 32.258064516129
88.4795643721843 35.4838709677419
104.004604226177 38.7096774193548
122.798701255813 41.9354838709677
147.63894643492 45.1612903225806
178.351306139555 48.3870967741936
218.659801237167 51.6129032258064
265.93619956933 54.8387096774194
329.779380995554 58.0645161290323
417.142489423725 61.2903225806452
546.059024116462 64.5161290322581
751.962918919328 67.741935483871
1131.60351242005 70.9677419354839
1820.04382746744 74.1935483870968
2994.17509603927 77.4193548387097
5231.88626543122 80.6451612903226
8504.47555976272 83.8709677419355
12377.9093633404 87.0967741935484
17205.8978355906 90.3225806451613
25155.1738731024 93.5483870967742
48353.1100398552 96.7741935483871
};
\addplot [thick, blue, dashed]
table {%
2.07877159706181 0
8.80121622131533 3.2258064516129
12.2441634926789 6.45161290322581
15.6739494174594 9.67741935483871
19.6287206058692 12.9032258064516
23.5993600401323 16.1290322580645
28.1684785904939 19.3548387096774
33.1060392950903 22.5806451612903
39.106505988132 25.8064516129032
44.7448623194989 29.0322580645161
51.2970485744789 32.258064516129
58.4474344108035 35.4838709677419
66.1937226917888 38.7096774193548
75.850358433536 41.9354838709677
86.1516360284942 45.1612903225806
97.2643563867118 48.3870967741936
109.508645716256 51.6129032258064
124.727132132913 54.8387096774194
143.092229856783 58.0645161290323
162.94987467542 61.2903225806452
187.902591498249 64.5161290322581
218.429824091449 67.741935483871
256.037074845428 70.9677419354839
305.591340370437 74.1935483870968
372.099931518562 77.4193548387097
471.45225715341 80.6451612903226
633.221979504409 83.8709677419355
945.113413518893 87.0967741935484
1666.13242848839 90.3225806451613
3876.39680170257 93.5483870967742
23909.9539634832 96.7741935483871
};

==> figures/raw_data/load_balancing/ptimes_mape.tex <==
\addplot[solid, green!70!black, thick, mark=none] table {%
15.1526089156341 0
15.1631279945016 1.78571428571429
15.1831686779329 3.57142857142857
15.3010849726636 5.35714285714286
15.4126471890709 7.14285714285714
15.6129758268833 8.92857142857143
16.0230819907382 10.7142857142857
21.9206955024511 12.5
21.9397050805521 14.2857142857143
21.999174629433 16.0714285714286
22.0238473261667 17.8571428571429
22.0478475072223 19.6428571428571
22.066790730084 21.4285714285714
22.0698929586209 23.2142857142857
22.2177076285149 25
22.2274181453327 26.7857142857143
22.2301465955787 28.5714285714286
22.2582110110259 30.3571428571429
22.2701916170277 32.1428571428571
22.2726026242095 33.9285714285714
22.3103594319139 35.7142857142857
22.3441756514609 37.5
22.3487826451824 39.2857142857143
22.659369813179 41.0714285714286
22.6916598700891 42.8571428571429
22.7308483714304 44.6428571428571
23.0006920848462 46.4285714285714
23.9861661848871 48.2142857142857
24.3500064999309 50
24.8566438452596 51.7857142857143
26.3447088121864 53.5714285714286
26.4218505472401 55.3571428571429
26.4625437317642 57.1428571428571
27.3014516176001 58.9285714285714
27.8754905509133 60.7142857142857
28.8611166976362 62.5
29.2957941474728 64.2857142857143
29.5559114182824 66.0714285714286
29.655228876883 67.8571428571429
29.9849496495963 69.6428571428571
30.5585616086408 71.4285714285714
30.8148111970194 73.2142857142857
30.9436715672784 75
32.3031946445336 76.7857142857143
33.2264591232814 78.5714285714286
33.9822347304487 80.3571428571429
34.4173897121063 82.1428571428571
34.4386056089752 83.9285714285714
34.8569752294749 85.7142857142857
43.4405875381654 87.5
43.5077020329616 89.2857142857143
43.6743960160688 91.0714285714286
44.9992164357101 92.8571428571429
45.0865286116092 94.6428571428571
46.2604342965484 96.4285714285714
46.614280407968 98.2142857142857
};

\addplot[solid, red, thick, mark=none] 
table {%
9.77426124652321 0
14.002521163523 0.833333333333333
22.6367055984572 1.66666666666667
23.2154262710423 2.5
25.285893532797 3.33333333333333
27.0314651541494 4.16666666666667
32.2552255754903 5
32.7106115957239 5.83333333333333
33.1777027026525 6.66666666666667
34.3479205372877 7.5
35.1678132638737 8.33333333333333
36.1131270149662 9.16666666666667
36.6320892518755 10
37.0224085297569 10.8333333333333
37.6155171233494 11.6666666666667
38.5866219930542 12.5
41.401131352116 13.3333333333333
41.8878928182454 14.1666666666667
42.5137949677324 15
43.8669842218944 15.8333333333333
51.244335981256 16.6666666666667
51.81363565078 17.5
52.6421172668468 18.3333333333333
53.3636401560879 19.1666666666667
54.7886645451583 20
55.3463607913973 20.8333333333333
56.5363876565606 21.6666666666667
57.554352106854 22.5
61.3626095741467 23.3333333333333
63.1126482271612 24.1666666666667
64.9877159273236 25
66.2079832779892 25.8333333333333
67.8148955573303 26.6666666666667
68.4402322069847 27.5
70.4707064788389 28.3333333333333
71.1087296058383 29.1666666666667
71.1423733739467 30
73.3770757300337 30.8333333333333
74.772035664815 31.6666666666667
82.4787147359017 32.5
86.0922369869254 33.3333333333333
88.9222261168237 34.1666666666667
91.5287309743355 35
91.7474926453447 35.8333333333333
92.7967356860947 36.6666666666667
94.2948751106288 37.5
97.3531845996316 38.3333333333333
97.7510306417445 39.1666666666667
102.13138313323 40
102.21343801205 40.8333333333333
102.9136943476 41.6666666666667
107.510311084988 42.5
109.08509973098 43.3333333333333
112.535831327228 44.1666666666667
114.799013343723 45
115.137770996408 45.8333333333333
119.021960317912 46.6666666666667
122.817804739974 47.5
122.958093066939 48.3333333333333
123.864970597345 49.1666666666667
124.642551735345 50
127.823952070226 50.8333333333333
132.958934174545 51.6666666666667
133.278261120031 52.5
133.803194574805 53.3333333333333
136.782931209336 54.1666666666667
137.527210418253 55
138.352870035644 55.8333333333333
138.355194254448 56.6666666666667
142.641330241209 57.5
142.782285150573 58.3333333333333
144.059363646561 59.1666666666667
144.976971050132 60
147.82417588219 60.8333333333333
148.103592558723 61.6666666666667
152.67083022396 62.5
154.696628285974 63.3333333333333
160.173326053675 64.1666666666667
161.891461039793 65
168.835484166315 65.8333333333333
170.048856927487 66.6666666666667
172.047155887544 67.5
177.839165531932 68.3333333333333
178.09365151202 69.1666666666667
178.452703386503 70
179.369954842354 70.8333333333333
182.76908534004 71.6666666666667
183.139719070513 72.5
184.721107317808 73.3333333333333
185.709719704017 74.1666666666667
189.05252762767 75
197.815470809887 75.8333333333333
204.48978608023 76.6666666666667
204.874831690782 77.5
212.818937762281 78.3333333333333
216.858165711365 79.1666666666667
226.359166057473 80
234.114778884069 80.8333333333333
238.763649806082 81.6666666666667
247.689958586748 82.5
262.007214225097 83.3333333333333
265.1828280884 84.1666666666667
271.368791967879 85
304.940959175397 85.8333333333333
313.824294702589 86.6666666666667
314.109437288989 87.5
338.509919302995 88.3333333333333
346.816868698781 89.1666666666667
364.120064797578 90
367.221467380008 90.8333333333333
379.310509893658 91.6666666666667
402.282026013074 92.5
426.896311163248 93.3333333333333
434.62922924192 94.1666666666667
441.380493688477 95
492.0155650236 95.8333333333333
503.897576979813 96.6666666666667
514.206586715059 97.5
577.789952927396 98.3333333333333
595.713688334687 99.1666666666667
};


==> figures/raw_data/load_balancing/ptimes_pol.tex <==
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\addplot[solid, green!70!black, thick, mark=none] 
table {%
-6.02319570954097 0
8.31905927311909 3.2258064516129
12.4998067309032 6.45161290322581
16.6532586897454 9.67741935483871
20.2259309526931 12.9032258064516
23.7649240967233 16.1290322580645
27.8193265830701 19.3548387096774
32.6456370839801 22.5806451612903
38.0032860641079 25.8064516129032
43.728278995621 29.0322580645161
50.2365030631091 32.258064516129
56.9585182775361 35.4838709677419
64.5524162100138 38.7096774193548
72.712493906572 41.9354838709677
81.6405251733252 45.1612903225806
91.1553495450841 48.3870967741936
101.98462269521 51.6129032258064
113.546242830769 54.8387096774194
127.247840508508 58.0645161290323
142.924243633878 61.2903225806452
159.340177612462 64.5161290322581
177.32568244958 67.741935483871
195.698661231706 70.9677419354839
217.245355279267 74.1935483870968
244.210088287819 77.4193548387097
282.578519546947 80.6451612903226
337.38908031308 83.8709677419355
416.370266526889 87.0967741935484
545.867122043024 90.3225806451613
772.436455327975 93.5483870967742
1766.93411101925 96.7741935483871
};
\addplot [thick, red, solid]
table {%
2.11116951586348 0
10.9045527376192 3.2258064516129
15.1438591661502 6.45161290322581
19.8958688140835 9.67741935483871
24.9083794051582 12.9032258064516
30.4273209674117 16.1290322580645
36.5637026447875 19.3548387096774
42.8573151107077 22.5806451612903
49.2318202794859 25.8064516129032
56.7257094646822 29.0322580645161
64.626455268106 32.258064516129
74.254944917565 35.4838709677419
83.6754757647705 38.7096774193548
94.44020730395 41.9354838709677
105.416554848578 45.1612903225806
119.067717122541 48.3870967741936
133.944771012563 51.6129032258064
150.160612161862 54.8387096774194
168.192476638539 58.0645161290323
188.690065625214 61.2903225806452
213.137909305845 64.5161290322581
240.039806289972 67.741935483871
276.479136766175 70.9677419354839
318.854590508396 74.1935483870968
373.20919884122 77.4193548387097
446.66021691844 80.6451612903226
546.667258501115 83.8709677419355
673.782146338335 87.0967741935484
856.173991084065 90.3225806451613
1136.9100175619 93.5483870967742
2378.48831413708 96.7741935483871
};
\addplot[dashed, blue, thick, mark=none]
table {%
2.07877159706181 0
8.69740951503235 3.2258064516129
12.1094166819896 6.45161290322581
15.4526199416901 9.67741935483871
19.3273357550653 12.9032258064516
23.2007211797969 16.1290322580645
27.6770698017575 19.3548387096774
32.382985728791 22.5806451612903
38.0996521538848 25.8064516129032
43.5357982729438 29.0322580645161
49.5400950922465 32.258064516129
56.2457457453206 35.4838709677419
63.2426519800422 38.7096774193548
71.5576377630376 41.9354838709677
80.8938199012905 45.1612903225806
90.7969607452574 48.3870967741936
100.513979569292 51.6129032258064
112.239259429328 54.8387096774194
125.708532759005 58.0645161290323
140.94499406386 61.2903225806452
155.941529270731 64.5161290322581
173.945203673208 67.741935483871
193.478476788096 70.9677419354839
217.003440870597 74.1935483870968
245.693039450959 77.4193548387097
286.479654128767 80.6451612903226
336.390097330008 83.8709677419355
416.261721318793 87.0967741935484
555.877782683545 90.3225806451613
795.567711602374 93.5483870967742
1985.7538003133 96.7741935483871
};
